PLGC: Pseudo-Labeled Graph Condensation

Large graph datasets make training graph neural networks (GNNs) computationally costly. Graph condensation methods address this by generating small synthetic graphs that approximate the original data. However, existing approaches rely on clean, supervised labels, which limits their reliability when labels are scarce, noisy, or inconsistent. We propose Pseudo-Labeled Graph Condensation (PLGC), a self-supervised framework that constructs latent pseudo-labels from node embeddings and optimizes condensed graphs to match the original graph's structural and feature statistics -- without requiring ground-truth labels. PLGC offers three key contributions: (1) A diagnosis of why supervised condensation fails under label noise and distribution shift. (2) A label-free condensation method that jointly learns latent prototypes and node assignments. (3) Theoretical guarantees showing that pseudo-labels preserve latent structural statistics of the original graph and ensure accurate embedding alignment. Empirically, across node classification and link prediction tasks, PLGC achieves competitive performance with state-of-the-art supervised condensation methods on clean datasets and exhibits substantial robustness under label noise, often outperforming all baselines by a significant margin. Our findings highlight the practical and theoretical advantages of self-supervised graph condensation in noisy or weakly-labeled environments.

==> sections/abstract.tex <==
% Graph condensation reduces the size of large-scale graphs, optimizing memory usage and computational efficiency while maintaining performance in downstream tasks. However, most existing methods rely on supervised learning with large amounts of labeled data, rendering them almost ineffective in scenarios with limited node labels or noisy data.
% To address these limitations, we introduce a novel self-supervised approach called \textit{Pseudo-Labeled Graph Condensation (PLGC)}. 
% In particular, PLGC generates synthetic node-level pseudo-labels by leveraging self-supervised latent node embeddings to create a condensed graph, eliminating the reliance on labeled data and hence, improving robustness in noisy environments.
% Through extensive experiments for node classification and link prediction, we demonstrate the superiority of our PLGC method that not only ensures stable and robust performance in presence of node level label noise, but also produce comparable performance with the existing supervised techniques in presence of $100\%$ clean labels for their condensation.\footnote{Code Link: \href{https://anonymous.4open.science/r/PLGC-0B26/}{https://anonymous.4open.science/r/PLGC-0B26/}}



% \keywords{Graph Condensation  \and Self Supervision \and Graph Neural Nets \and Label Noise \and Node Classification \and Link Prediction}
% \end{abstract}


Large graph datasets make training graph neural networks (GNNs) computationally costly. Graph condensation methods address this by generating small synthetic graphs that approximate the original data. However, existing approaches rely on clean, supervised labels, which limits their reliability when labels are scarce, noisy, or inconsistent.
We propose Pseudo-Labeled Graph Condensation (PLGC), a self-supervised framework that constructs latent pseudo-labels from node embeddings and optimizes condensed graphs to match the original graph’s structural and feature statistics—without requiring ground-truth labels.
PLGC offers three key contributions: (1) A diagnosis of why supervised condensation fails under label noise and distribution shift. (2) A label-free condensation method that jointly learns latent prototypes and node assignments. (3) Theoretical guarantees showing that pseudo-labels preserve latent structural statistics of the original graph and ensure accurate embedding alignment.
Empirically, across node classification and link prediction tasks, PLGC achieves competitive performance with state-of-the-art supervised condensation methods on clean datasets and exhibits substantial robustness under label noise, often outperforming all baselines by a significant margin. 
Our findings highlight the practical and theoretical advantages of self-supervised graph condensation in noisy or weakly-labeled environments. \footnote{Code Link: \href{https://anonymous.4open.science/r/PLGC-0B26/}{https://anonymous.4open.science/r/PLGC-0B26/}}



